An Output Sensitive Algorithm for Discrete Convex Hulls

$\def\DD{{{\bf \delta}}}\def\CH{{\mathop{\mathrm{ConvexHull}}}}\newcommand{\LL}{{\cal {L}}} \newcommand{\ZZ}{\mathbb{Z}} $ Given a convex body $C$ in the plane, its discrete hull is $C^0 = \CH( C \cap \LL )$, where $\LL = \ZZ \times \ZZ$ is the integer lattice. We present an $O( |C^0| \log \DD(C) )$-time algorithm for calculating the discrete hull of $C$, where $|C^0|$ denotes the number of vertices of $C^0$, and $\DD(C)$ is the diameter of $C$. Actually, using known combinatorial bounds, the running time of the algorithm is $O(\DD(C)^{2/3} \log{\DD(C)})$. In particular, this bound applies when $C$ is a disk.

==> figs/t1.tex <==
%
%
%
\centering
\begin{tabular}{|r||r|r|r||r|r|r||}
\cline{2-7}
\multicolumn{1}{c||}{} &\multicolumn{3}{c||}{Points on $DH$} & \multicolumn{3}{c||}{$|DH|/r^{2/3}$} \\
\hline
$r$ & Min & Max & Avg. & Min & Max & Avg. \\
\hline
\hline
10 & 15 & 20 & 16 & 3.750 & 5.000 & 4.143 \\
100 & 68 & 85 & 74 & 3.238 & 4.048 & 3.555 \\
1,000 & 333 & 360 & 345 & 3.330 & 3.600 & 3.450 \\
10,000 & 1,568 & 1,636 & 1,603 & 3.379 & 3.526 & 3.456 \\
100,000 & 7,355 & 7,521 & 7,442 & 3.415 & 3.492 & 3.455 \\
1,000,000 & 34,358 & 34,720 & 34,535 & 3.436 & 3.472 & 3.454 \\
10,000,000 & 159,879 & 160,674 & 160,317 & 3.445 & 3.462 & 3.454 \\
\hline
\end{tabular}
%
%
%


==> figs/t2.tex <==
%
%
%
\centering
\begin{tabular}{|r||r|r|r||r|r|r||}
\cline{2-7}
\multicolumn{1}{c||}{} &\multicolumn{3}{c||}{Points on $DHS$} & \multicolumn{3}{c||}{$|DHS|/r^{2/3}$} \\
\hline
$r$ & Min & Max & Avg. & Min & Max & Avg. \\
\hline
\hline
10 & 32 & 46 & 40 & 8.000 & 11.500 & 10.123 \\
100 & 216 & 251 & 235 & 10.286 & 11.952 & 11.216 \\
1,000 & 1,075 & 1,278 & 1,217 & 10.750 & 12.780 & 12.173 \\
10,000 & 5,697 & 6,260 & 5,986 & 12.278 & 13.491 & 12.902 \\
100,000 & 28,081 & 29,748 & 28,807 & 13.037 & 13.811 & 13.374 \\
1,000,000 & 133,964 & 139,767 & 137,535 & 13.396 & 13.977 & 13.754 \\
10,000,000 & 637,281 & 657,949 & 647,339 & 13.730 & 14.175 & 13.947 \\
\hline
\end{tabular}
%
%
%


==> figs/t3.tex <==
%
%
%
\centering
\begin{tabular}{|r||r|r|r|r|}
%
%
%
%
\cline{2-5}
\multicolumn{1}{c||}{} & \multicolumn{1}{c|}{Avg. Number of Points} &
 \multicolumn{1}{c|}{Max. Number of} &
 \multicolumn{2}{c|}{Time in Seconds} \\
%
\cline{1-1}\cline{4-5}$r$ & \multicolumn{1}{c|}{on Discrete Hull} &  
 \multicolumn{1}{c|}{Iterations Per Edge} 
 & DCH & IG \\
\hline
\hline
10 & 16 & 5 & 0.0015 & 0.0010 \\
100 & 74 & 6 & 0.0097 & 0.0097 \\
1,000 & 345 & 7 & 0.0550 & 0.0890 \\
10,000 & 1,603 & 9 & 0.2935 & 0.8991 \\
100,000 & 7,442 & 11 & 1.5259 & 9.0403 \\
1,000,000 & 34,535 & 13 & 7.9662 & 90.4785 \\
10,000,000 & 160,317 & 14 & 43.0855 & 906.9861 \\
\hline
\end{tabular}
%
%
%


==> figs/tbl_gcd.tex <==
%
%
%
\centering
\begin{tabular}{||r|r||l|l||r||}
%
\hline
~ & ~ & ~ & 
Representation  &
 The \hspace{1.5cm} 
~\\ 
{$a$}  &
%
 {$b$}  & {$\floor{{a}/{b}}$} & 
{of $ ( 14, 31 ) $} & 
{ convergent $ r_i $ } %
%
\\\hline
$ 31 $  &  $ 14 $  &  $ 2 $ & $ 31 (0, 1) + 14 (1, 0) $ &
        $2\bigr.$
\\ %
$ 14 $  &  $ 3 $  &  $ 4 $ & $ 14 (1, 2) + 3 (0, 1) $ &
        $2 + \frac{1}{4\bigr.}$
\\ %
$ 3 $  &  $ 2 $  &  $ 1 $ & $ 3 (4, 9) + 2 (1, 2) $ &
        $2 + \frac{1}{4 + \frac{1}{1\bigr.}}$
\\ %
$ 2 $  &  $ 1 $  &  $ 2 $ & $ 2 (5, 11) + 1 (4, 9) $ &
        $2 + \frac{1}{4 + \frac{1}{1 + \frac{1}{2\bigr.}}}$
\\ %
\hline
\end{tabular}

%
%
%

